On the generation of periodic discrete structures with identical two-point correlation

Strategies for the generation of periodic discrete structures with identical two-point correlation are developed. Starting from a pair of root structures, which are not related by translation, phase inversion or axis reflections, child structures of arbitrary resolution (i.e., pixel or voxel numbers) and number of phases (i.e., material phases/species) can be generated by means of trivial embedding based phase extension, application of kernels and/or phase coalescence, such that the generated structures inherit the two-point-correlation equivalence. Proofs of the inheritance property are provided by means of the Discrete Fourier Transform theory. A Python 3 implementation of the results is offered by the authors through the Github repository https://github.com/DataAnalyticsEngineering/EQ2PC in order to make the provided results reproducible and useful for all interested readers. Examples for the generation of structures are demonstrated, together with applications in the homogenization theory of periodic media.

==> macros_mf2.tex <==
\usepackage{amsmath} % \boldsymbol, \mathcal, \mathbf, \mathrm, \mathsf, \mathtt 
\usepackage{amssymb} % \mathbb, \mathfrak 
%\usepackage{undertilde} % \utilde
\usepackage[mathscr]{eucal} % \mathscr
\DeclareMathAlphabet{\mathda}{OT1}{pzc}{m}{it} % needed for declaring an alphabet

% Whatever
\newcommand{\norm}[1]{{\| #1 \|}}
\newcommand{\eps}{\varepsilon}

% Operators
\newcommand{\grad}{\mathrm{grad}}
\renewcommand{\div}{\mathrm{div}}
\newcommand{\sym}{\mathrm{sym}}

% Sets
\newcommand{\so}{\mathsf{SO(3)}}

% Fonts
\newcommand{\ua}{\underline{a}}
\newcommand{\ub}{\underline{b}}
\newcommand{\uc}{\underline{c}}
\newcommand{\ud}{\underline{d}}
\newcommand{\ue}{\underline{e}}
\newcommand{\uf}{\underline{f}}
\newcommand{\ug}{\underline{g}}
\newcommand{\uh}{\underline{h}}
\newcommand{\ui}{\underline{i}}
\newcommand{\uj}{\underline{j}}
\newcommand{\uk}{\underline{k}}
\newcommand{\ul}{\underline{l}}
\newcommand{\um}{\underline{m}}
\newcommand{\un}{\underline{n}}
\newcommand{\uo}{\underline{o}}
\newcommand{\up}{\underline{p}}
\newcommand{\uq}{\underline{q}}
\newcommand{\ur}{\underline{r}}
\newcommand{\us}{\underline{s}}
\newcommand{\ut}{\underline{t}}
\newcommand{\uu}{\underline{u}}
\newcommand{\uv}{\underline{v}}
\newcommand{\uw}{\underline{w}}
\newcommand{\ux}{\underline{x}}
\newcommand{\uy}{\underline{y}}
\newcommand{\uz}{\underline{z}}

\newcommand{\uA}{\underline{A}}
\newcommand{\uB}{\underline{B}}
\newcommand{\uC}{\underline{C}}
\newcommand{\uD}{\underline{D}}
\newcommand{\uE}{\underline{E}}
\newcommand{\uF}{\underline{F}}
\newcommand{\uG}{\underline{G}}
\newcommand{\uH}{\underline{H}}
\newcommand{\uI}{\underline{I}}
\newcommand{\uJ}{\underline{J}}
\newcommand{\uK}{\underline{K}}
\newcommand{\uL}{\underline{L}}
\newcommand{\uM}{\underline{M}}
\newcommand{\uN}{\underline{N}}
\newcommand{\uO}{\underline{O}}
\newcommand{\uP}{\underline{P}}
\newcommand{\uQ}{\underline{Q}}
\newcommand{\uR}{\underline{R}}
\newcommand{\uS}{\underline{S}}
\newcommand{\uT}{\underline{T}}
\newcommand{\uU}{\underline{U}}
\newcommand{\uV}{\underline{V}}
\newcommand{\uW}{\underline{W}}
\newcommand{\uX}{\underline{X}}
\newcommand{\uY}{\underline{Y}}
\newcommand{\uZ}{\underline{Z}}

%\newcommand{\utA}{\utilde{A}}
%\newcommand{\utB}{\utilde{B}}
%\newcommand{\utC}{\utilde{C}}
%\newcommand{\utD}{\utilde{D}}
%\newcommand{\utE}{\utilde{E}}
%\newcommand{\utF}{\utilde{F}}
%\newcommand{\utG}{\utilde{G}}
%\newcommand{\utH}{\utilde{H}}
%\newcommand{\utI}{\utilde{I}}
%\newcommand{\utJ}{\utilde{J}}
%\newcommand{\utK}{\utilde{K}}
%\newcommand{\utL}{\utilde{L}}
%\newcommand{\utM}{\utilde{M}}
%\newcommand{\utN}{\utilde{N}}
%\newcommand{\utO}{\utilde{O}}
%\newcommand{\utP}{\utilde{P}}
%\newcommand{\utQ}{\utilde{Q}}
%\newcommand{\utR}{\utilde{R}}
%\newcommand{\utS}{\utilde{S}}
%\newcommand{\utT}{\utilde{T}}
%\newcommand{\utU}{\utilde{U}}
%\newcommand{\utV}{\utilde{V}}
%\newcommand{\utW}{\utilde{W}}
%\newcommand{\utX}{\utilde{X}}
%\newcommand{\utY}{\utilde{Y}}
%\newcommand{\utZ}{\utilde{Z}}

\newcommand{\uuA}{\underline{\underline{A}}}
\newcommand{\uuB}{\underline{\underline{B}}}
\newcommand{\uuC}{\underline{\underline{C}}}
\newcommand{\uuD}{\underline{\underline{D}}}
\newcommand{\uuE}{\underline{\underline{E}}}
\newcommand{\uuF}{\underline{\underline{F}}}
\newcommand{\uuG}{\underline{\underline{G}}}
\newcommand{\uuH}{\underline{\underline{H}}}
\newcommand{\uuI}{\underline{\underline{I}}}
\newcommand{\uuJ}{\underline{\underline{J}}}
\newcommand{\uuK}{\underline{\underline{K}}}
\newcommand{\uuL}{\underline{\underline{L}}}
\newcommand{\uuM}{\underline{\underline{M}}}
\newcommand{\uuN}{\underline{\underline{N}}}
\newcommand{\uuO}{\underline{\underline{O}}}
\newcommand{\uuP}{\underline{\underline{P}}}
\newcommand{\uuQ}{\underline{\underline{Q}}}
\newcommand{\uuR}{\underline{\underline{R}}}
\newcommand{\uuS}{\underline{\underline{S}}}
\newcommand{\uuT}{\underline{\underline{T}}}
\newcommand{\uuU}{\underline{\underline{U}}}
\newcommand{\uuV}{\underline{\underline{V}}}
\newcommand{\uuW}{\underline{\underline{W}}}
\newcommand{\uuX}{\underline{\underline{X}}}
\newcommand{\uuY}{\underline{\underline{Y}}}
\newcommand{\uuZ}{\underline{\underline{Z}}}

\newcommand{\ualpha}{\underline{\alpha}}
\newcommand{\ubeta}{\underline{\beta}}
\newcommand{\ugamma}{\underline{\gamma}}
\newcommand{\udelta}{\underline{\delta}}
\newcommand{\uepsilon}{\underline{\epsilon}}
\newcommand{\uzeta}{\underline{\zeta}}
\newcommand{\ueta}{\underline{\eta}}
\newcommand{\utheta}{\underline{\theta}}
\newcommand{\uiota}{\underline{\iota}}
\newcommand{\ukappa}{\underline{\kappa}}
\newcommand{\ulambda}{\underline{\lambda}}
\newcommand{\umu}{\underline{\mu}}
\newcommand{\unu}{\underline{\nu}}
\newcommand{\uxi}{\underline{\xi}}
\newcommand{\uomicron}{\underline{\omicron}}
\newcommand{\upi}{\underline{\pi}}
\newcommand{\urho}{\underline{\rho}}
\newcommand{\usigma}{\underline{\sigma}}
\newcommand{\utau}{\underline{\tau}}
\newcommand{\uupsilon}{\underline{\upsilon}}
\newcommand{\uphi}{\underline{\phi}}
\newcommand{\uchi}{\underline{\chi}}
\newcommand{\upsi}{\underline{\psi}}
\newcommand{\uomega}{\underline{\omega}}
\newcommand{\uvarepsilon}{\underline{\varepsilon}}
\newcommand{\uvartheta}{\underline{\vartheta}}
\newcommand{\uvarphi}{\underline{\varphi}}
\newcommand{\usig}{\usigma}
\newcommand{\ueps}{\uvarepsilon}

\newcommand{\uAlpha}{\underline{\Alpha}}
\newcommand{\uBeta}{\underline{\Beta}}
\newcommand{\uGamma}{\underline{\Gamma}}
\newcommand{\uDelta}{\underline{\Delta}}
\newcommand{\uEpsilon}{\underline{\Epsilon}}
\newcommand{\uZeta}{\underline{\Zeta}}
\newcommand{\uEta}{\underline{\Eta}}
\newcommand{\uTheta}{\underline{\Theta}}
\newcommand{\uIota}{\underline{\Iota}}
\newcommand{\uKappa}{\underline{\Kappa}}
\newcommand{\uLambda}{\underline{\Lambda}}
\newcommand{\uMu}{\underline{\Mu}}
\newcommand{\uNu}{\underline{\Nu}}
\newcommand{\uXi}{\underline{\Xi}}
\newcommand{\uOmicron}{\underline{\Omicron}}
\newcommand{\uPi}{\underline{\Pi}}
\newcommand{\uRho}{\underline{\Rho}}
\newcommand{\uSigma}{\underline{\Sigma}}
\newcommand{\uTau}{\underline{\Tau}}
\newcommand{\uUpsilon}{\underline{\Upsilon}}
\newcommand{\uPhi}{\underline{\Phi}}
\newcommand{\uChi}{\underline{\Chi}}
\newcommand{\uPsi}{\underline{\Psi}}
\newcommand{\uOmega}{\underline{\Omega}}

\newcommand{\uuAlpha}{\underline{\underline{\Alpha}}}
\newcommand{\uuBeta}{\underline{\underline{\Beta}}}
\newcommand{\uuGamma}{\underline{\underline{\Gamma}}}
\newcommand{\uuDelta}{\underline{\underline{\Delta}}}
\newcommand{\uuEpsilon}{\underline{\underline{\Epsilon}}}
\newcommand{\uuZeta}{\underline{\underline{\Zeta}}}
\newcommand{\uuEta}{\underline{\underline{\Eta}}}
\newcommand{\uuTheta}{\underline{\underline{\Theta}}}
\newcommand{\uuIota}{\underline{\underline{\Iota}}}
\newcommand{\uuKappa}{\underline{\underline{\Kappa}}}
\newcommand{\uuLambda}{\underline{\underline{\Lambda}}}
\newcommand{\uuMu}{\underline{\underline{\Mu}}}
\newcommand{\uuNu}{\underline{\underline{\Nu}}}
\newcommand{\uuXi}{\underline{\underline{\Xi}}}
\newcommand{\uuOmicron}{\underline{\underline{\Omicron}}}
\newcommand{\uuPi}{\underline{\underline{\Pi}}}
\newcommand{\uuRho}{\underline{\underline{\Rho}}}
\newcommand{\uuSigma}{\underline{\underline{\Sigma}}}
\newcommand{\uuTau}{\underline{\underline{\Tau}}}
\newcommand{\uuUpsilon}{\underline{\underline{\Upsilon}}}
\newcommand{\uuPhi}{\underline{\underline{\Phi}}}
\newcommand{\uuChi}{\underline{\underline{\Chi}}}
\newcommand{\uuPsi}{\underline{\underline{\Psi}}}
\newcommand{\uuOmega}{\underline{\underline{\Omega}}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\ba}{\boldsymbol{a}}
\newcommand{\bb}{\boldsymbol{b}}
\newcommand{\bc}{\boldsymbol{c}}
\newcommand{\bd}{\boldsymbol{d}}
\newcommand{\be}{\boldsymbol{e}}
\newcommand{\bff}{\boldsymbol{f}}
\newcommand{\bg}{\boldsymbol{g}}
\newcommand{\bh}{\boldsymbol{h}}
\newcommand{\bi}{\boldsymbol{i}}
\newcommand{\bj}{\boldsymbol{j}}
\newcommand{\bk}{\boldsymbol{k}}
\newcommand{\bl}{\boldsymbol{l}}
\newcommand{\bm}{\boldsymbol{m}}
\newcommand{\bn}{\boldsymbol{n}}
\newcommand{\bo}{\boldsymbol{o}}
\newcommand{\bp}{\boldsymbol{p}}
\newcommand{\bq}{\boldsymbol{q}}
\newcommand{\br}{\boldsymbol{r}}
\newcommand{\bs}{\boldsymbol{s}}
\newcommand{\bt}{\boldsymbol{t}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bz}{\boldsymbol{z}}

\newcommand{\bA}{\boldsymbol{A}}
\newcommand{\bB}{\boldsymbol{B}}
\newcommand{\bC}{\boldsymbol{C}}
\newcommand{\bD}{\boldsymbol{D}}
\newcommand{\bE}{\boldsymbol{E}}
\newcommand{\bF}{\boldsymbol{F}}
\newcommand{\bG}{\boldsymbol{G}}
\newcommand{\bH}{\boldsymbol{H}}
\newcommand{\bI}{\boldsymbol{I}}
\newcommand{\bJ}{\boldsymbol{J}}
\newcommand{\bK}{\boldsymbol{K}}
\newcommand{\bL}{\boldsymbol{L}}
\newcommand{\bM}{\boldsymbol{M}}
\newcommand{\bN}{\boldsymbol{N}}
\newcommand{\bO}{\boldsymbol{O}}
\newcommand{\bP}{\boldsymbol{P}}
\newcommand{\bQ}{\boldsymbol{Q}}
\newcommand{\bR}{\boldsymbol{R}}
\newcommand{\bS}{\boldsymbol{S}}
\newcommand{\bT}{\boldsymbol{T}}
\newcommand{\bU}{\boldsymbol{U}}
\newcommand{\bV}{\boldsymbol{V}}
\newcommand{\bW}{\boldsymbol{W}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\bZ}{\boldsymbol{Z}}

\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}
\newcommand{\bzeta}{\boldsymbol{\zeta}}
\newcommand{\betaa}{\boldsymbol{\eta}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\biota}{\boldsymbol{\iota}}
\newcommand{\bkappa}{\boldsymbol{\kappa}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bnu}{\boldsymbol{\nu}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bomicron}{\boldsymbol{\omicron}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\brho}{\boldsymbol{\rho}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\btau}{\boldsymbol{\tau}}
\newcommand{\bupsilon}{\boldsymbol{\upsilon}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bchi}{\boldsymbol{\chi}}
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\bomega}{\boldsymbol{\omega}}
\newcommand{\bvarepsilon}{\boldsymbol{\varepsilon}}
\newcommand{\bvartheta}{\boldsymbol{\vartheta}}
\newcommand{\bvarphi}{\boldsymbol{\varphi}}

\newcommand{\bAlpha}{\boldsymbol{\Alpha}}
\newcommand{\bBeta}{\boldsymbol{\Beta}}
\newcommand{\bGamma}{\boldsymbol{\Gamma}}
\newcommand{\bDelta}{\boldsymbol{\Delta}}
\newcommand{\bEpsilon}{\boldsymbol{\Epsilon}}
\newcommand{\bZeta}{\boldsymbol{\Zeta}}
\newcommand{\bEta}{\boldsymbol{\Eta}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\bIota}{\boldsymbol{\Iota}}
\newcommand{\bKappa}{\boldsymbol{\Kappa}}
\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\bMu}{\boldsymbol{\Mu}}
\newcommand{\bNu}{\boldsymbol{\Nu}}
\newcommand{\bXi}{\boldsymbol{\Xi}}
\newcommand{\bOmicron}{\boldsymbol{\Omicron}}
\newcommand{\bPi}{\boldsymbol{\Pi}}
\newcommand{\bRho}{\boldsymbol{\Rho}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\bTau}{\boldsymbol{\Tau}}
\newcommand{\bUpsilon}{\boldsymbol{\Upsilon}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bChi}{\boldsymbol{\Chi}}
\newcommand{\bPsi}{\boldsymbol{\Psi}}
\newcommand{\bOmega}{\boldsymbol{\Omega}}

\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}

\newcommand{\sfa}{\mathsf{a}}
\newcommand{\sfb}{\mathsf{b}}
\newcommand{\sfc}{\mathsf{c}}
\newcommand{\sfd}{\mathsf{d}}
\newcommand{\sfe}{\mathsf{e}}
\newcommand{\sff}{\mathsf{f}}
\newcommand{\sfg}{\mathsf{g}}
\newcommand{\sfh}{\mathsf{h}}
\newcommand{\sfi}{\mathsf{i}}
\newcommand{\sfj}{\mathsf{j}}
\newcommand{\sfk}{\mathsf{k}}
\newcommand{\sfl}{\mathsf{l}}
\newcommand{\sfm}{\mathsf{m}}
\newcommand{\sfn}{\mathsf{n}}
\newcommand{\sfo}{\mathsf{o}}
\newcommand{\sfp}{\mathsf{p}}
\newcommand{\sfq}{\mathsf{q}}
\newcommand{\sfr}{\mathsf{r}}
\newcommand{\sfs}{\mathsf{s}}
\newcommand{\sft}{\mathsf{t}}
\newcommand{\sfu}{\mathsf{u}}
\newcommand{\sfv}{\mathsf{v}}
\newcommand{\sfw}{\mathsf{w}}
\newcommand{\sfx}{\mathsf{x}}
\newcommand{\sfy}{\mathsf{y}}
\newcommand{\sfz}{\mathsf{z}}

\newcommand{\sfA}{\mathsf{A}}
\newcommand{\sfB}{\mathsf{B}}
\newcommand{\sfC}{\mathsf{C}}
\newcommand{\sfD}{\mathsf{D}}
\newcommand{\sfE}{\mathsf{E}}
\newcommand{\sfF}{\mathsf{F}}
\newcommand{\sfG}{\mathsf{G}}
\newcommand{\sfH}{\mathsf{H}}
\newcommand{\sfI}{\mathsf{I}}
\newcommand{\sfJ}{\mathsf{J}}
\newcommand{\sfK}{\mathsf{K}}
\newcommand{\sfL}{\mathsf{L}}
\newcommand{\sfM}{\mathsf{M}}
\newcommand{\sfN}{\mathsf{N}}
\newcommand{\sfO}{\mathsf{O}}
\newcommand{\sfP}{\mathsf{P}}
\newcommand{\sfQ}{\mathsf{Q}}
\newcommand{\sfR}{\mathsf{R}}
\newcommand{\sfS}{\mathsf{S}}
\newcommand{\sfT}{\mathsf{T}}
\newcommand{\sfU}{\mathsf{U}}
\newcommand{\sfV}{\mathsf{V}}
\newcommand{\sfW}{\mathsf{W}}
\newcommand{\sfX}{\mathsf{X}}
\newcommand{\sfY}{\mathsf{Y}}
\newcommand{\sfZ}{\mathsf{Z}}

\newcommand{\rma}{\mathrm{a}}
\newcommand{\rmb}{\mathrm{b}}
\newcommand{\rmc}{\mathrm{c}}
\newcommand{\rmd}{\mathrm{d}}
\newcommand{\rme}{\mathrm{e}}
\newcommand{\rmf}{\mathrm{f}}
\newcommand{\rmg}{\mathrm{g}}
\newcommand{\rmh}{\mathrm{h}}
\newcommand{\rmi}{\mathrm{i}}
\newcommand{\rmj}{\mathrm{j}}
\newcommand{\rmk}{\mathrm{k}}
\newcommand{\rml}{\mathrm{l}}
\newcommand{\rmm}{\mathrm{m}}
\newcommand{\rmn}{\mathrm{n}}
\newcommand{\rmo}{\mathrm{o}}
\newcommand{\rmp}{\mathrm{p}}
\newcommand{\rmq}{\mathrm{q}}
\newcommand{\rmr}{\mathrm{r}}
\newcommand{\rms}{\mathrm{s}}
\newcommand{\rmt}{\mathrm{t}}
\newcommand{\rmu}{\mathrm{u}}
\newcommand{\rmv}{\mathrm{v}}
\newcommand{\rmw}{\mathrm{w}}
\newcommand{\rmx}{\mathrm{x}}
\newcommand{\rmy}{\mathrm{y}}
\newcommand{\rmz}{\mathrm{z}}

\newcommand{\rmA}{\mathrm{A}}
\newcommand{\rmB}{\mathrm{B}}
\newcommand{\rmC}{\mathrm{C}}
\newcommand{\rmD}{\mathrm{D}}
\newcommand{\rmE}{\mathrm{E}}
\newcommand{\rmF}{\mathrm{F}}
\newcommand{\rmG}{\mathrm{G}}
\newcommand{\rmH}{\mathrm{H}}
\newcommand{\rmI}{\mathrm{I}}
\newcommand{\rmJ}{\mathrm{J}}
\newcommand{\rmK}{\mathrm{K}}
\newcommand{\rmL}{\mathrm{L}}
\newcommand{\rmM}{\mathrm{M}}
\newcommand{\rmN}{\mathrm{N}}
\newcommand{\rmO}{\mathrm{O}}
\newcommand{\rmP}{\mathrm{P}}
\newcommand{\rmQ}{\mathrm{Q}}
\newcommand{\rmR}{\mathrm{R}}
\newcommand{\rmS}{\mathrm{S}}
\newcommand{\rmT}{\mathrm{T}}
\newcommand{\rmU}{\mathrm{U}}
\newcommand{\rmV}{\mathrm{V}}
\newcommand{\rmW}{\mathrm{W}}
\newcommand{\rmX}{\mathrm{X}}
\newcommand{\rmY}{\mathrm{Y}}
\newcommand{\rmZ}{\mathrm{Z}}
